Signal recovery in the polychromatic computed tomography model: Injectivity and complexity

We consider a nonlinear model motivated by polychromatic computed tomography (CT). Here, $W$ distinct $d$-dimensional signals $x^*_1, \ldots, x^*_W \in \mathbb{R}^d$ must be recovered from $n$ measurements $(a_i, y_i)_{i = 1}^n$ that obey the nonlinear model $\mathbb{E}[y_i|a_i] = h(\langle a_i, x^*_1 \rangle, \ldots, \langle a_i, x^*_W \rangle)$, where $h: \mathbb{R}^W \to \mathbb{R}$ is a known nonlinearity that models a certain type of exponential attenuation law. Even when there is no noise in the measurements, the sample size $n$ (for any measurement ensemble $\{a_i\}_{i = 1}^n$) must exceed the number of unknowns $Wd$ to guarantee that the underlying signals are identifiable. We construct a measurement ensemble that ensures perfect signal recovery almost surely provided $n \geq Wd + W - 1$, thereby isolating the injectivity threshold up to an additive factor $W - 1$. We also study computational complexity of signal recovery in this model with a general measurement ensemble $\{a_i\}$. We show that if $W \geq 2$, then there is a measurement ensemble for which deciding whether there exist signals consistent with the measurements is NP-hard. In particular, this implies that polychromatic, multimaterial CT reconstruction is NP-hard in general. This finding stands in sharp contrast to the single-material setting, for which a polynomial-time algorithm can provably perform signal recovery for any measurement ensemble.

==> commands-mm.tex <==
%!TEX root = main-paper-template.tex

% The command above makes the PDF compilable from this file if you're using SublimeText

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Some basic packages
\usepackage{setspace}
\usepackage{indentfirst}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\xccomment}[1]{{\bf{{\red{{XC --- #1}}}}}}


\usepackage{comment}
\usepackage{epsf}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{bbm}
\usepackage{color}
\usepackage{nicefrac}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath, bm}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amssymb}
\usepackage{textcomp}
\usepackage{adjustbox}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage[ruled, vlined, lined, commentsnumbered]{algorithm2e}
% \documentclass{article}

\RequirePackage[colorlinks,citecolor={blue!60!black},urlcolor={blue!70!black},linkcolor={red!60!black},breaklinks,hypertexnames=false]{hyperref} %Adds links to references (without boxes)
\usepackage{cleveref}
\usepackage{stmaryrd}

% Alternative minipage environment, renders better in terms of spacing

\newenvironment{fminipage}%
  {\begin{Sbox}\begin{minipage}}%
  {\end{minipage}\end{Sbox}\fbox{\TheSbox}}
  
\newenvironment{algbox}[0]{\vskip 0.2in
\noindent 
\begin{fminipage}{6.3in}
}{
\end{fminipage}
\vskip 0.2in
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS BELOW

%%%%%%%


\newcommand{\algname}{\textrm{EXACT}}




% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper, not by section number and not combined


\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{claim}{Claim}
\newtheorem{Condition}{C}

%%%%%%%%%%%
%References (natbib): Use \citet and \citep to take full advantage

% \usepackage{natbib}
% \setcitestyle{round}

%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Widebar command
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
 \settowidth{\widebarargwidth}{\ensuremath{#1}}%
 \settoheight{\widebarargheight}{\ensuremath{#1}}%
 \settodepth{\widebarargdepth}{\ensuremath{#1}}%
 \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
 \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
 \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
   \hspace{0.3\widebarargdepth}%
   \addtolength{\widebarargheight}{0.3ex}%
   \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
 {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
       \vskip 0.8ex
       \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
       \parindent 1.5em 
       \dimen0=\hsize
       \advance\dimen0 by -3em
       \ifdim \wd\@tempboxa >\dimen0
               \hbox to \hsize{
                       \parindent 0em
                       \hfil 
                       \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                               {\bf #1.} #2
                               %%\unhbox\@tempboxa
                               } 
                       \hfil}
       \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
       \fi
       }
\makeatother



%% COMMENTING commands: insert more for more than two collaborators

\long\def\comment#1{}

\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\apcomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}

\newcommand{\green}[1]{\textcolor{OliveGreen!80}{#1}}
\newcommand{\kavcomment}[1]{{\bf{{\green{{KAV --- #1}}}}}}

\newcommand{\mqcomment}[1]{{\bf{{\red{{MQ --- #1}}}}}}

\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\sfkcomment}[1]{{\bf{{\purple{{SFK --- #1}}}}}}


% Some vector/matrix norms. Convention is that we use triple lines for matrix 
% norms and double lines for vector norms.
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

% Some useful and common operators
% Independence symbol
\newcommand\indpt{\protect\mathpalette{\protect\independenT}{\perp}} 
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\defn}{\coloneqq} %This is a properly aligned definition symbol
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\dist}{\rho}
\DeclareMathOperator{\trace}{\mathsf{tr}}



% Specific norms
\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{F}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}
\newcommand{\eucnorm}[1]{\left\|#1 \right\|}
\newcommand{\linfnorm}[1]{\left\|#1 \right\|_\infty}
\newcommand{\op}{\mathsf{op}}

% Bracket notation to make life easier when writing long expressions
\newcommand{\paren}[1]{\left\{ #1 \right\} }
% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}
\newcommand{\llangle}{\langle\!\langle}
\newcommand{\rrangle}{\rangle\!\rangle}
\newcommand{\trinprod}[2]{\ensuremath{\llangle #1 , \, #2 \rrangle}}

% The macros below are useful if you see these quantities changing over the course of writing
\newcommand{\numdim}{\ensuremath{d}}
\newcommand{\numobs}{\ensuremath{n}}

% Distances between distributions
\newcommand{\kull}[2]{\ensuremath{D_{\mathsf{KL}}(#1\; \| \; #2)}}
\newcommand{\KL}{\ensuremath{D_{\mathsf{KL}}}}
\newcommand{\TV}{\ensuremath{d_{\mathsf{TV}}}}
\newcommand{\Hel}{\ensuremath{d_{\mathsf{hel}}}}

% Probability
\newcommand{\EE}{\ensuremath{{\mathbb{E}}}}
%\newcommand{\Prob}{\ensuremath{{\Partition}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}
\newcommand{\ind}[1]{\ensuremath{{\mathbb{I}\left\{ #1 \right\}}}}

%Numbering (use with \overset to label steps)
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
\newcommand{\6}{\ensuremath{{\sf (vi)}}}

%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}


% Distributions
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}

% Script letters
\newcommand{\Aspace}{\ensuremath{\mathcal{A}}}
\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}
\newcommand{\real}{\mathbb{R}}

% Population and sample loss functions
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\lossn}[1]{\ensuremath{\mathcal{L}^n \left( #1 \right)}}

% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimates
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}
\newcommand{\thetabar}{\ensuremath{\overline{\theta}}}
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

% Order notation
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\ordertil}{\ensuremath{\widetilde{\order}}}
\newcommand{\Omegatil}{\ensuremath{\widetilde{\Omega}}}

% Vectors and matrices
\newcommand{\bI}{\boldsymbol{I}}

% Macros for monotone CT
\newcommand{\monotone}{\nu}
\newcommand{\norm}{\|x_{\star}\|_{2}}
\newcommand{\N}{W}
\newcommand{\coeff}{\mu}
\newcommand{\Photon}{\widebar{I}}

% Macros for blind deconvolution
\newcommand{\polylog}{\log^{6}(d)}
\newcommand{\Err}{\mathsf{Err}}
\newcommand{\Errdet}{\mathsf{Err}^{\mathsf{det}}}
\newcommand{\parcompZ}{\widetilde{\alpha}}
\newcommand{\parcompdetZ}{\widetilde{\alpha}^{\mathsf{det}}}
\newcommand{\parcompseqZ}{\widetilde{\alpha}^{\mathsf{seq}}}
\newcommand{\perpcompZ}{\widetilde{\beta}}
\newcommand{\perpcompdetZ}{\widetilde{\beta}^{\mathsf{det}}}
\newcommand{\perpcompseqZ}{\widetilde{\beta}^{\mathsf{seq}}}
\newcommand{\parcompX}{\alpha}
\newcommand{\parcompdetX}{\alpha^{\mathsf{det}}}
\newcommand{\parcompseqX}{\alpha^{\mathsf{seq}}}
\newcommand{\perpcompX}{\beta}
\newcommand{\perpcompdetX}{\beta^{\mathsf{det}}}
\newcommand{\perpcompseqX}{\beta^{\mathsf{seq}}}
\newcommand{\iotaX}{\iota}
\newcommand{\iotadetX}{\iota^{\mathsf{det}}}
\newcommand{\iotaZ}{\widetilde{\iota}}
\newcommand{\iotadetZ}{\widetilde{\iota}^{\mathsf{det}}}
\newcommand{\etaX}{\eta}
\newcommand{\etadetX}{\eta^{\mathsf{det}}}
\newcommand{\etaZ}{\widetilde{\eta}}
\newcommand{\etadetZ}{\widetilde{\eta}^{\mathsf{det}}}
\newcommand{\oversamp}{\Lambda}
\newcommand{\lambdamax}{\lambda_{\mathsf{max}}}

\newcommand{\lambdamin}{\lambda_{\mathsf{min}}}

\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bWtil}{\widetilde{\boldsymbol{W}}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bSig}{\boldsymbol{\Sigma}}
\newcommand{\perpX}{\beta}
\newcommand{\parX}{\alpha}
\newcommand{\perpZ}{\iota}
\newcommand{\parZ}{\gamma}
\newcommand{\coefX}{\mu}
\newcommand{\bcoefX}{\boldsymbol{\mu}}
\newcommand{\coefZ}{\nu}
\newcommand{\bcoefZ}{\boldsymbol{\nu}}
\newcommand{\epsilondn}{\epsilon_{d,n}}
\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\Cdm}{C_{d,m}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bO}{\boldsymbol{O}}
\newcommand{\dev}{\frac{1}{\lambda\sqrt{n}}}
\newcommand{\thetaXdet}{\theta^{\mathsf{det}}}
\newcommand{\thetaZdet}{\widetilde{\theta}^{\mathsf{det}}}
\newcommand{\thetaX}{\theta}
\newcommand{\thetaZ}{\widetilde{\theta}}
\newcommand{\LZ}{\widetilde{L}}
\newcommand{\GZ}{\widetilde{G}}
\newcommand{\alphaXmap}{F}
\newcommand{\alphaZmap}{\widetilde{F}}
\newcommand{\iotaXmap}{H}
\newcommand{\iotaZmap}{\widetilde{H}}
\newcommand{\etaXmap}{S}
\newcommand{\etaZmap}{\widetilde{S}}
\newcommand{\detstatemap}{\mathcal{T}}
\newcommand{\prox}{\mathcal{G}_{m,\lambda}}
\newcommand{\R}{\mathbb{R}}


% Vector, matrix, mathcal, and mathbb macros
\newcommand{\va}{\bm{a}}
\newcommand{\vb}{\bm{b}}
\newcommand{\vc}{\bm{c}}
\newcommand{\vd}{\bm{d}}
\newcommand{\ve}{\bm{e}}
\newcommand{\vf}{\bm{f}}
\newcommand{\vg}{\bm{g}}
\newcommand{\vh}{\bm{h}}
\newcommand{\vu}{\bm{u}}
\newcommand{\vv}{\bm{v}}
\newcommand{\vx}{\bm{x}}
\newcommand{\vy}{\bm{y}}
\newcommand{\vz}{\bm{z}}
\newcommand{\vr}{\bm{r}}
\newcommand{\vm}{\bm{m}}
\newcommand{\vn}{\bm{n}}
\newcommand{\vs}{\bm{s}}
\newcommand{\vxi}{\bm{\xi}}
\newcommand{\vomega}{\bm{\omega}}
\newcommand{\vgamma}{\bm{\gamma}}
\newcommand{\vzero}{\bm{0}}
\newcommand{\vone}{\bm{1}}
\newcommand{\vdelta}{\bm{\delta}}
\newcommand{\vmu}{\bm{\mu}}
\newcommand{\vzeta}{\bm{\zeta}}
\newcommand{\ones}{\bm{1}}
\let\vecone\ones
\newcommand{\vw}{\bm{w}}
\newcommand{\valpha}{\bm{\alpha}}
\newcommand{\vlambda}{\bm{\lambda}}
\newcommand{\vtheta}{\bm{\theta}}


% Leave one out notation
\newcommand{\Xcol}[1]{\bX^{(#1)}}
\newcommand{\Xloco}[1]{\bX_{\backslash #1}}
\newcommand{\coefXloco}[1]{\widehat{\coefX}^{(\backslash#1)}}
\newcommand{\Constant}{16}

